Subcritical Turbulence in the Mega Ampere Spherical Tokamak

The transport of heat out of tokamak plasmas by turbulence is the dominant mechanism limiting the performance of fusion reactors. Turbulence can be driven by the ion temperature gradient (ITG) and suppressed by toroidal sheared flows. Numerical simulations attempting to understand turbulence are crucial for guiding the design of future reactors. We investigate ion-scale turbulence via gyrokinetic simulations in the outer core of the Mega Ampere Spherical Tokamak (MAST). We perform a parameter scan in the values of the ITG and the flow shear. We show that nonlinear simulations reproduce the experimental ion heat flux and that the experimental values of the ITG and the flow shear lie close to the turbulence threshold. We demonstrate that the system is subcritical in the presence of flow shear, i.e., the system is formally stable, but transitions to a turbulent state given a large enough initial perturbation. We propose a scenario for the transition to turbulence previously unreported in tokamak plasmas: close to the threshold, the plasma is dominated by a low number of coherent long-lived structures; as the system is taken away from the threshold into the more unstable regime, the number of these structures increases until they fill the domain and a more conventional turbulence emerges. We make comparisons of correlation properties between our simulations and experimental measurements of density fluctuations from the MAST BES diagnostic. We apply a synthetic diagnostic to our simulation data and find reasonable agreement of the correlation properties of the simulated and experimental turbulence, most notably of the correlation time. We show that the properties of turbulence are essentially functions of the ion heat flux. We find that turbulence close to the threshold is strongly affected by flow shear, whereas far from threshold, the turbulence resembles a conventional ITG-driven regime.

==> dedication.tex <==
\begin{acknowledgements}
To all those who failed to stop me going into academia, damn youuuuuu!
\end{acknowledgements}


==> titlepage.tex <==
\title{\thetitle}
\date{\theyear}
\author{\theauthor}


\maketitle

